Social Network Integration: Towards Constructing the Social Graph

In this work, we formulate the problem of social network integration. It takes multiple observed social networks as input and returns an integrated global social graph where each node corresponds to a real person. The key challenge for social network integration is to discover the correspondences or interlinks across different social networks. We engaged an in-depth analysis across three online social networks, AMiner, Linkedin, and Videolectures in order to address what reveals users' social identity, whether the social factors consistent across different social networks and how we can leverage these information to perform integration. We proposed a unified framework for the social network integration task. It crawls data from multiple social networks and further discovers accounts correspond to the same real person from the obtained networks. We use a probabilistic model to determine such correspondence, it incorporates features like the consistency of social status and social ties across different, as well as one-to-one mapping constraint and logical transitivity to jointly make the prediction. Empirical experiments verify the effectiveness of our method.

==> expsetup.tex <==
\section{Experimental Setup}
\label{sec:expsetup}

\vpara{Prediction Setting}
We use the data set described in \S \ref{sec:observe}. To compare the performance of our proposed model with alternative methods, we carefully select a sub cross domain described in Table \ref{tab:statistics} from the data set, which all the authors have some cross domain collaboration and some research experience, i.e., each user has at least five publications over more than one domain. We divided all the publications into 16 time stamps by viewing every year as time setup.

Our goal is to predict whether a user will have a cross domain collaboration next time stamp. But after we make some analysis about all the publications, we find that it is difficult to use the same year to predict the all kind of cross domains collaboration. Some use different part of time for each cross domain. And we use the first 10 time stamps to for training and predicate collaboration in following 6 time stamps.

\vpara{Comparison Methods} We prepare the following methods to compare with the proposed approach:

\indent
\vpara{Content Homophily(CH):} It use the users' content homophily to recommend the cross domain collaboration. We trained the several parameters to calculate all the content based similarity, then recommend the candidates to user.

\indent
\vpara{Social Ties(ST):} It use a common sense that if two people have some kind of relationships(even cross some body else), they may have more probability to know each other. It use the social ties, common neighbors, structural balance theory.

\indent
\vpara{Ties \& Content(TC):} it consider the influence both content homophily and social ties and make a linear exploration objective function which combine them.

\indent
\vpara{PreFG:} the proposed approach, which use a factor graph model with all features.

In the four methods, the content homophily considers structural homophily, research homophily and geographic distance factors. Social Ties uses link homophily and structural balance factors. PreFG and Ties \& Content considers all factors we defined.

\vpara{Evaluation Measures} To evaluate the performance of different, we use Precision(P): P@5, P@10, P@15, P@20 and Average Precision(AP).

\indent
All codes are implemented in C++ and JAVA, and all the evaluations are performed on an x64 machine with E7520 1.87GHz Intel Xeon CPU and 128G RAM. The operation system is Microsoft Windows Sever 2008 R2 Enterprise. All methods have a good efficiency performance: the CPU time needed for prediction by all algorithm on the all the cross domains. The training time for all methods with ranges 1 to 4 minutes.


==> survey.tex <==
\section{Survey}
\label{sec:survey}

\textbf{A Bayesian Method for Matching Two Similar Graphs without Seeds}

This paper proposed a Bayesian method for approximate graph matching. It based on a generative model that treats the two observable graphs as independent samples of a fixed underlying generator graph. Based on this approach, they derive the probability that a mapping between a pair of nodes is correct given their evidence.

Exact graph matching: equivalent to the graph isomorphism problem (or exact subgraph matching). The goal is to find a edge-preserving node mapping. A variation of this problem finds an almost correct node mapping between the graphs using statistical methods, such as random works [7], expectation maximization [9], and the Bayesian edit-distance[10].
